BIPEFT: Budget-Guided Iterative Search for Parameter Efficient Fine-Tuning of Large Pretrained Language Models

Parameter Efficient Fine-Tuning (PEFT) offers an efficient solution for fine-tuning large pretrained language models for downstream tasks. However, most PEFT strategies are manually designed, often resulting in suboptimal performance. Recent automatic PEFT approaches aim to address this but face challenges such as search space entanglement, inefficiency, and lack of integration between parameter budgets and search processes. To overcome these issues, we introduce a novel Budget-guided Iterative search strategy for automatic PEFT (BIPEFT), significantly enhancing search efficiency. BIPEFT employs a new iterative search strategy to disentangle the binary module and rank dimension search spaces. Additionally, we design early selection strategies based on parameter budgets, accelerating the learning process by gradually removing unimportant modules and fixing rank dimensions. Extensive experiments on public benchmarks demonstrate the superior performance of BIPEFT in achieving efficient and effective PEFT for downstream tasks with a low parameter budget.

==> 3_preliminary_analysis.tex <==
\section{Preliminary Analysis}
\subsection{Idea}
\subsubsection{Motivation}

\subsubsection{Challenges}



==> 5.0_search_space.tex <==
\subsection{Search Space and Experiments Settings}
\label{sec:setting}




Generally, we will follow the search space settings of those baselines for fair comparison. \\

For NLP task, although different baselines all report the results on GLUE and SuperGLUE, they have various search space and experiments settings. Since the search method we designed is flexible, we will follow the original settings of these baselines instead of changing the original settings for better comparison.\\
\textbf{$S^3$Delta}: This method uses $\text{T5}_{\text{large}}$ (703M parameters) as the backbone. It designs two search space settings. 
\begin{itemize}
    \item \textbf{LoRA}. They narrow down the search space into a single type of PEFT module and choose LoRA as an example. The position search space is same with that in vision experiments setting.
    \item \textbf{Mix}. It contains a mixture of LoRA, Adapter-LR, Bitfit, and LNFIT modules. Following $S^3$Delta, we limit Adapter-LR to the outputs of the attention module and the feedforward layer in a transformer layer. For BitFit, the potential applied positions are all the linear modules (Q, K, V, O, W1, W2) and the Layer Normalization modules (LN). For LNFit, the potential positions are all the LN modules. We denote this setting as MoM-S.
\end{itemize}

\textbf{AutoPEFT}: This work uses $\text{BERT}_{\text{base}}$ as the backbone and conducted per-task search on GLUE. It combines Serial Adapters (SA), Parallel Adapters (PA), and Prefix-Tuning (PT) as the three representative modules in the search space. We denote this setting as MoM-A.

Pruning based method are also used to search for PEFT architectures ~\cite{lawton-etal-2023-neural}. This method search for PEFT based on LoRA and BitFit and reports the seach result on RoBERTa-large on GLUE development set. We list our results under the same search space and backbone in Appendix \ref{appendix:1}.
